Centralization in Proof-of-Stake Blockchains: A Game-Theoretic Analysis of Bootstrapping Protocols

Proof-of-stake (PoS) has emerged as a natural alternative to the resource-intensive Proof-of-Work (PoW) blockchain, as was recently seen with the Ethereum Merge. PoS-based blockchains require an initial stake distribution among the participants. Typically, this initial stake distribution is called bootstrapping. This paper argues that existing bootstrapping protocols are prone to centralization. To address centralization due to bootstrapping, we propose a novel game $\Gamma_\textsf{bootstrap}$. Next, we define three conditions: (i) Individual Rationality (IR), (ii) Incentive Compatibility (IC), and (iii) $(\tau,\delta,\epsilon)-$ Decentralization that an \emph{ideal} bootstrapping protocol must satisfy. $(\tau,\delta,\epsilon)$ are certain parameters to quantify decentralization. Towards this, we propose a novel centralization metric, C-NORM, to measure centralization in a PoS System. We define a centralization game -- $\Gamma_\textsf{cent}$, to analyze the efficacy of centralization metrics. We show that C-NORM effectively captures centralization in the presence of strategic players capable of launching Sybil attacks. With C-NORM, we analyze popular bootstrapping protocols such as Airdrop and Proof-of-Burn (PoB) and prove that they do not satisfy IC and IR, respectively. Motivated by the Ethereum Merge, we study W2SB (a PoW-based bootstrapping protocol) and prove it is ideal. In addition, we conduct synthetic simulations to empirically validate that W2SB bootstrapped PoS is decentralized.

==> references.tex <==
%%% -*-BibTeX-*-
%%% Do NOT edit. File created by BibTeX with style
%%% ACM-Reference-Format-Journals [18-Jan-2012].

\begin{thebibliography}{65}

    %%% ====================================================================
    %%% NOTE TO THE USER: you can override these defaults by providing
    %%% customized versions of any of these macros before the \bibliography
    %%% command.  Each of them MUST provide its own final punctuation,
    %%% except for \shownote{}, \showDOI{}, and \showURL{}.  The latter two
    %%% do not use final punctuation, in order to avoid confusing it with
    %%% the Web address.
    %%%
    %%% To suppress output of a particular field, define its macro to expand
    %%% to an empty string, or better, \unskip, like this:
    %%%
    %%% \newcommand{\showDOI}[1]{\unskip}   % LaTeX syntax
    %%%
    %%% \def \showDOI #1{\unskip}           % plain TeX syntax
    %%%
    %%% ====================================================================
    
    \ifx \showCODEN    \undefined \def \showCODEN     #1{\unskip}     \fi
    \ifx \showDOI      \undefined \def \showDOI       #1{#1}\fi
    \ifx \showISBNx    \undefined \def \showISBNx     #1{\unskip}     \fi
    \ifx \showISBNxiii \undefined \def \showISBNxiii  #1{\unskip}     \fi
    \ifx \showISSN     \undefined \def \showISSN      #1{\unskip}     \fi
    \ifx \showLCCN     \undefined \def \showLCCN      #1{\unskip}     \fi
    \ifx \shownote     \undefined \def \shownote      #1{#1}          \fi
    \ifx \showarticletitle \undefined \def \showarticletitle #1{#1}   \fi
    \ifx \showURL      \undefined \def \showURL       {\relax}        \fi
    % The following commands are used for tagged output and should be
    % invisible to TeX
    \providecommand\bibfield[2]{#2}
    \providecommand\bibinfo[2]{#2}
    \providecommand\natexlab[1]{#1}
    \providecommand\showeprint[2][]{arXiv:#2}
    
    \bibitem[\protect\citeauthoryear{??}{mar}{2023}]%
            {marketcap}
     \bibinfo{year}{2023}\natexlab{}.
    \newblock \bibinfo{title}{CoinMarketCap}.
    \newblock \bibinfo{howpublished}{\url{coinmarketcap.com/ }}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Alkalay-Houlihan and Shah}{Alkalay-Houlihan
      and Shah}{2019}]%
            {blockchainPoA}
    \bibfield{author}{\bibinfo{person}{Colleen Alkalay-Houlihan} {and}
      \bibinfo{person}{Nisarg Shah}.} \bibinfo{year}{2019}\natexlab{}.
    \newblock \showarticletitle{The Pure Price of Anarchy of Pool Block Withholding
      Attacks in Bitcoin Mining}. In \bibinfo{booktitle}{\emph{AAAI}}.
      \bibinfo{pages}{1724--1731}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Azouvi, Maller, and Meiklejohn}{Azouvi
      et~al\mbox{.}}{2018}]%
            {empericalGovernance}
    \bibfield{author}{\bibinfo{person}{Sarah Azouvi}, \bibinfo{person}{Mary
      Maller}, {and} \bibinfo{person}{Sarah Meiklejohn}.}
      \bibinfo{year}{2018}\natexlab{}.
    \newblock \showarticletitle{Egalitarian Society or Benevolent Dictatorship: The
      State of Cryptocurrency Governance}. In \bibinfo{booktitle}{\emph{Financial
      Cryptography Workshops}}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Becker, D'Angelo, and Gilbert}{Becker
      et~al\mbox{.}}{2021}]%
            {centralityShapley}
    \bibfield{author}{\bibinfo{person}{Ruben Becker}, \bibinfo{person}{Gianlorenzo
      D'Angelo}, {and} \bibinfo{person}{Hugo Gilbert}.}
      \bibinfo{year}{2021}\natexlab{}.
    \newblock \showarticletitle{Maximizing Influence-Based Group Shapley
      Centrality}. In \bibinfo{booktitle}{\emph{AAMAS}}.
      \bibinfo{pages}{1461–1463}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Bitcoinwhoswho}{Bitcoinwhoswho}{2018}]%
            {PoBResource1}
    \bibfield{author}{\bibinfo{person}{Bitcoinwhoswho}.}
      \bibinfo{year}{2018}\natexlab{}.
    \newblock \bibinfo{title}{~2 BTC BURNED IN 2018}.
    \newblock
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{BitcoinWiki}{BitcoinWiki}{2018}]%
            {PoBResource2}
    \bibfield{author}{\bibinfo{person}{BitcoinWiki}.}
      \bibinfo{year}{2018}\natexlab{}.
    \newblock \bibinfo{title}{Proof of burn}.
    \newblock
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Buterin et~al\mbox{.}}{Buterin
      et~al\mbox{.}}{[n.d.]}]%
            {buterin2013ethereum}
    \bibfield{author}{\bibinfo{person}{Vitalik Buterin} {et~al\mbox{.}}}
      \bibinfo{year}{[n.d.]}\natexlab{}.
    \newblock \bibinfo{title}{Ethereum white paper}.
    \newblock
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Castro and Liskov}{Castro and Liskov}{1999}]%
            {Castro1999pBFT}
    \bibfield{author}{\bibinfo{person}{Miguel Castro} {and}
      \bibinfo{person}{Barbara Liskov}.} \bibinfo{year}{1999}\natexlab{}.
    \newblock \showarticletitle{Practical Byzantine fault tolerance}. In
      \bibinfo{booktitle}{\emph{Proceedings of the Third Symposium on Operating
      Systems Design and Implementation}} (New Orleans, Louisiana, USA)
      \emph{(\bibinfo{series}{OSDI '99})}. \bibinfo{publisher}{USENIX Association},
      \bibinfo{address}{USA}, \bibinfo{pages}{173–186}.
    \newblock
    \showISBNx{1880446391}
    
    
    \bibitem[\protect\citeauthoryear{Chong}{Chong}{2023}]%
            {AirdropResource2}
    \bibfield{author}{\bibinfo{person}{Julie-Anne Chong}.}
      \bibinfo{year}{2023}\natexlab{}.
    \newblock \bibinfo{title}{OpenDAO Airdrops SOS on OpenSea Community}.
    \newblock
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Chung and Shi}{Chung and Shi}{2023}]%
            {elaineShiTFM}
    \bibfield{author}{\bibinfo{person}{Hao Chung} {and} \bibinfo{person}{Elaine
      Shi}.} \bibinfo{year}{2023}\natexlab{}.
    \newblock \showarticletitle{Foundations of transaction fee mechanism design}.
      In \bibinfo{booktitle}{\emph{ACM-SIAM Symposium on Discrete Algorithms
      (SODA)}}. \bibinfo{pages}{3856--3899}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{David, Gazi, Kiayias, and Russell}{David
      et~al\mbox{.}}{2018}]%
            {posOuroboros2018}
    \bibfield{author}{\bibinfo{person}{Bernardo~Machado David},
      \bibinfo{person}{Peter Gazi}, \bibinfo{person}{Aggelos Kiayias}, {and}
      \bibinfo{person}{Alexander Russell}.} \bibinfo{year}{2018}\natexlab{}.
    \newblock \showarticletitle{Ouroboros Praos: An Adaptively-Secure,
      Semi-synchronous Proof-of-Stake Blockchain}. In
      \bibinfo{booktitle}{\emph{International Conference on the Theory and
      Application of Cryptographic Techniques}}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{de~Andres, Arroyo, Correia, and
      Rezola}{de~Andres et~al\mbox{.}}{2021}]%
            {challengesICO}
    \bibfield{author}{\bibinfo{person}{Pablo de Andres}, \bibinfo{person}{David
      Arroyo}, \bibinfo{person}{Ricardo Correia}, {and} \bibinfo{person}{{\'A}lvaro
      Rezola}.} \bibinfo{year}{2021}\natexlab{}.
    \newblock \showarticletitle{Challenges of the market for initial coin
      offerings}.
    \newblock \bibinfo{journal}{\emph{International Review of Financial Analysis}}
      (\bibinfo{year}{2021}).
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Douceur}{Douceur}{2002}]%
            {sybilAttack2002}
    \bibfield{author}{\bibinfo{person}{John~R. Douceur}.}
      \bibinfo{year}{2002}\natexlab{}.
    \newblock \showarticletitle{The Sybil Attack}. In
      \bibinfo{booktitle}{\emph{International Workshop on Peer-to-Peer Systems}}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Ethereum}{Ethereum}{2022}]%
            {ethereumMerge}
    \bibfield{author}{\bibinfo{person}{Ethereum}.} \bibinfo{year}{2022}\natexlab{}.
    \newblock \bibinfo{title}{The Merge}.
    \newblock
    \newblock
    \urldef\tempurl%
    \url{ethereum.org/en/upgrades/merge/}
    \showURL{%
    \tempurl}
    
    
    \bibitem[\protect\citeauthoryear{Fan, Min, Wu, and Cai}{Fan
      et~al\mbox{.}}{2023}]%
            {Airdrop}
    \bibfield{author}{\bibinfo{person}{Sizheng Fan}, \bibinfo{person}{Tian Min},
      \bibinfo{person}{Xiao Wu}, {and} \bibinfo{person}{Wei Cai}.}
      \bibinfo{year}{2023}\natexlab{}.
    \newblock \showarticletitle{Altruistic and Profit-Oriented: Making Sense of
      Roles in Web3 Community from Airdrop Perspective}. In
      \bibinfo{booktitle}{\emph{Proceedings of the 2023 CHI Conference on Human
      Factors in Computing Systems}} (Hamburg, Germany) \emph{(\bibinfo{series}{CHI
      '23})}. \bibinfo{publisher}{Association for Computing Machinery},
      \bibinfo{address}{New York, NY, USA}, Article \bibinfo{articleno}{551},
      \bibinfo{numpages}{16}~pages.
    \newblock
    \showISBNx{9781450394215}
    
    
    \bibitem[\protect\citeauthoryear{Foundation}{Foundation}{[n.d.]}]%
            {icon}
    \bibfield{author}{\bibinfo{person}{ICON Foundation}.}
      \bibinfo{year}{[n.d.]}\natexlab{}.
    \newblock \bibinfo{title}{ICON Blockchain}.
    \newblock
    \newblock
    \urldef\tempurl%
    \url{https://docs.icon.foundation/ICON-Whitepaper-EN-Draft.pdf}
    \showURL{%
    \tempurl}
    
    
    \bibitem[\protect\citeauthoryear{Garay, Kiayias, and Leonardos}{Garay
      et~al\mbox{.}}{2015}]%
            {backbone}
    \bibfield{author}{\bibinfo{person}{Juan Garay}, \bibinfo{person}{Aggelos
      Kiayias}, {and} \bibinfo{person}{Nikos Leonardos}.}
      \bibinfo{year}{2015}\natexlab{}.
    \newblock \showarticletitle{The Bitcoin Backbone Protocol: Analysis and
      Applications}. In \bibinfo{booktitle}{\emph{Advances in Cryptology -
      EUROCRYPT 2015}}, \bibfield{editor}{\bibinfo{person}{Elisabeth Oswald} {and}
      \bibinfo{person}{Marc Fischlin}} (Eds.). \bibinfo{publisher}{Springer Berlin
      Heidelberg}, \bibinfo{address}{Berlin, Heidelberg},
      \bibinfo{pages}{281--310}.
    \newblock
    \showISBNx{978-3-662-46803-6}
    
    
    \bibitem[\protect\citeauthoryear{Gervais, Karame, Capkun, and Capkun}{Gervais
      et~al\mbox{.}}{2014}]%
            {isBitcoinDecentralized}
    \bibfield{author}{\bibinfo{person}{Arthur Gervais}, \bibinfo{person}{Ghassan~O.
      Karame}, \bibinfo{person}{Vedran Capkun}, {and} \bibinfo{person}{Srdjan
      Capkun}.} \bibinfo{year}{2014}\natexlab{}.
    \newblock \showarticletitle{Is Bitcoin a Decentralized Currency?}
    \newblock \bibinfo{journal}{\emph{IEEE S\&P}}  \bibinfo{volume}{12}
      (\bibinfo{year}{2014}), \bibinfo{pages}{54--60}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Gilad, Hemo, Micali, Vlachos, and
      Zeldovich}{Gilad et~al\mbox{.}}{2017}]%
            {algorand}
    \bibfield{author}{\bibinfo{person}{Yossi Gilad}, \bibinfo{person}{Rotem Hemo},
      \bibinfo{person}{Silvio Micali}, \bibinfo{person}{Georgios Vlachos}, {and}
      \bibinfo{person}{Nickolai Zeldovich}.} \bibinfo{year}{2017}\natexlab{}.
    \newblock \showarticletitle{Algorand: Scaling Byzantine Agreements for
      Cryptocurrencies}.
    \newblock \bibinfo{journal}{\emph{Symposium on Operating Systems Principles}}
      (\bibinfo{year}{2017}), \bibinfo{pages}{51--68}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Gini}{Gini}{1921}]%
            {GiniCoeff}
    \bibfield{author}{\bibinfo{person}{Corrado Gini}.}
      \bibinfo{year}{1921}\natexlab{}.
    \newblock \showarticletitle{Measurement of Inequality of Incomes}.
    \newblock \bibinfo{journal}{\emph{The Economic Journal}}  \bibinfo{volume}{31}
      (\bibinfo{year}{1921}), \bibinfo{pages}{124}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Gochhayat, Shetty, Mukkamala, Foytik, Kamhoua,
      and Njilla}{Gochhayat et~al\mbox{.}}{2020}]%
            {gochhayatGini}
    \bibfield{author}{\bibinfo{person}{Sarada~Prasad Gochhayat},
      \bibinfo{person}{Sachin Shetty}, \bibinfo{person}{Ravi Mukkamala},
      \bibinfo{person}{Peter Foytik}, \bibinfo{person}{Georges~A. Kamhoua}, {and}
      \bibinfo{person}{Laurent Njilla}.} \bibinfo{year}{2020}\natexlab{}.
    \newblock \showarticletitle{Measuring Decentrality in Blockchain Based
      Systems}.
    \newblock \bibinfo{journal}{\emph{IEEE Access}}  \bibinfo{volume}{8}
      (\bibinfo{year}{2020}), \bibinfo{pages}{178372--178390}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Goodman}{Goodman}{2014}]%
            {tezos}
    \bibfield{author}{\bibinfo{person}{Lisl~Marburg Goodman}.}
      \bibinfo{year}{2014}\natexlab{}.
    \newblock \bibinfo{title}{Tezos : A Self-Amending Crypto-Ledger Position
      Paper}.
    \newblock
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Grossi}{Grossi}{2022}]%
            {DavideAAMAS22}
    \bibfield{author}{\bibinfo{person}{Davide Grossi}.}
      \bibinfo{year}{2022}\natexlab{}.
    \newblock \showarticletitle{Social Choice Around the Block: On the
      Computational Social Choice of Blockchain}. In
      \bibinfo{booktitle}{\emph{AAMAS}}. \bibinfo{pages}{1788–1793}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Guo, Gao, Mei, Zhao, and Yang}{Guo
      et~al\mbox{.}}{2019}]%
            {storageCentralization}
    \bibfield{author}{\bibinfo{person}{Zhaohui Guo}, \bibinfo{person}{Zhen Gao},
      \bibinfo{person}{Haojuan Mei}, \bibinfo{person}{Ming Zhao}, {and}
      \bibinfo{person}{Jinsheng Yang}.} \bibinfo{year}{2019}\natexlab{}.
    \newblock \showarticletitle{Design and Optimization for Storage Mechanism of
      the Public Blockchain Based on Redundant Residual Number System}.
    \newblock \bibinfo{journal}{\emph{IEEE Access}}  \bibinfo{volume}{7}
      (\bibinfo{year}{2019}), \bibinfo{pages}{98546--98554}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Harrigan, Shi, and Illum}{Harrigan
      et~al\mbox{.}}{2018}]%
            {AirdropPrivacy}
    \bibfield{author}{\bibinfo{person}{Martin Harrigan}, \bibinfo{person}{Lei Shi},
      {and} \bibinfo{person}{Jacob Illum}.} \bibinfo{year}{2018}\natexlab{}.
    \newblock \showarticletitle{Airdrops and Privacy: A Case Study in
      Cross-Blockchain Analysis}. In \bibinfo{booktitle}{\emph{2018 IEEE
      International Conference on Data Mining Workshops (ICDMW)}}.
      \bibinfo{pages}{63--70}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Istrate and Bonchis}{Istrate and
      Bonchis}{2022}]%
            {multiAgentCentralizationGame}
    \bibfield{author}{\bibinfo{person}{Gabriel Istrate} {and}
      \bibinfo{person}{Cosmin Bonchis}.} \bibinfo{year}{2022}\natexlab{}.
    \newblock \showarticletitle{Being Central on the Cheap: Stability in
      Heterogeneous Multiagent Centrality Games}. In
      \bibinfo{booktitle}{\emph{AAMAS}}. \bibinfo{pages}{651–659}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Istrate, Bonchis, and Gatina}{Istrate
      et~al\mbox{.}}{2020}]%
            {coalitionGTCentrality}
    \bibfield{author}{\bibinfo{person}{Gabriel Istrate}, \bibinfo{person}{Cosmin
      Bonchis}, {and} \bibinfo{person}{Claudiu Gatina}.}
      \bibinfo{year}{2020}\natexlab{}.
    \newblock \showarticletitle{It's Not Whom You Know, It's What You, or Your
      Friends, Can Do: Coalitional Frameworks for Network Centralities}. In
      \bibinfo{booktitle}{\emph{AAMAS}}. \bibinfo{pages}{566–574}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Jia, Xu, Wu, Feng, Chen, and Yang}{Jia
      et~al\mbox{.}}{2022}]%
            {decentralizationMeasure}
    \bibfield{author}{\bibinfo{person}{Yongpu Jia}, \bibinfo{person}{Changqiao Xu},
      \bibinfo{person}{Zhonghui Wu}, \bibinfo{person}{Zichen Feng},
      \bibinfo{person}{Yaxin Chen}, {and} \bibinfo{person}{Shujie Yang}.}
      \bibinfo{year}{2022}\natexlab{}.
    \newblock \showarticletitle{Measuring Decentralization in Emerging Public
      Blockchains}. In \bibinfo{booktitle}{\emph{2022 International Wireless
      Communications and Mobile Computing (IWCMC)}}. \bibinfo{pages}{137--141}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Johnston, Thorsen, Liu, Kuebler, and
      Torrellas}{Johnston et~al\mbox{.}}{2018}]%
            {smartdropArticle}
    \bibfield{author}{\bibinfo{person}{David~A Johnston}, \bibinfo{person}{Mark
      Thorsen}, \bibinfo{person}{Henry Liu}, \bibinfo{person}{Erik Kuebler}, {and}
      \bibinfo{person}{Grace Torrellas}.} \bibinfo{year}{2018}\natexlab{}.
    \newblock \bibinfo{title}{The Smartdrop Model: How To Bootstrap Dapps and
      Protocols Without An ICO}.
    \newblock
    \newblock
    \urldef\tempurl%
    \url{djohnstonec.medium.com/the-smartdrop-model-859888916d94}
    \showURL{%
    \tempurl}
    
    
    \bibitem[\protect\citeauthoryear{Kapengut and Mizrach}{Kapengut and
      Mizrach}{2023}]%
            {energyMerge}
    \bibfield{author}{\bibinfo{person}{Elie Kapengut} {and} \bibinfo{person}{Bruce
      Mizrach}.} \bibinfo{year}{2023}\natexlab{}.
    \newblock \showarticletitle{An event study of the ethereum transition to
      proof-of-stake}.
    \newblock \bibinfo{journal}{\emph{Commodities}} \bibinfo{volume}{2},
      \bibinfo{number}{2} (\bibinfo{year}{2023}), \bibinfo{pages}{96--110}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Karakostas, Kiayias, and Zacharias}{Karakostas
      et~al\mbox{.}}{2023}]%
            {kiayiasNash}
    \bibfield{author}{\bibinfo{person}{Dimitris Karakostas},
      \bibinfo{person}{Aggelos Kiayias}, {and} \bibinfo{person}{Thomas Zacharias}.}
      \bibinfo{year}{2023}\natexlab{}.
    \newblock \showarticletitle{Blockchain Nash Dynamics and the Pursuit of
      Compliance}. In \bibinfo{booktitle}{\emph{Proceedings of the 4th ACM
      Conference on Advances in Financial Technologies}} (Cambridge, MA, USA)
      \emph{(\bibinfo{series}{AFT '22})}. \bibinfo{publisher}{Association for
      Computing Machinery}, \bibinfo{address}{New York, NY, USA},
      \bibinfo{pages}{281–293}.
    \newblock
    \showISBNx{9781450398619}
    \urldef\tempurl%
    \url{https://doi.org/10.1145/3558535.3559781}
    \showDOI{\tempurl}
    
    
    \bibitem[\protect\citeauthoryear{Karantias, Kiayias, and Zindros}{Karantias
      et~al\mbox{.}}{2020}]%
            {PoB2020}
    \bibfield{author}{\bibinfo{person}{Kostis Karantias}, \bibinfo{person}{Aggelos
      Kiayias}, {and} \bibinfo{person}{Dionysis Zindros}.}
      \bibinfo{year}{2020}\natexlab{}.
    \newblock \showarticletitle{Proof-of-Burn}. In
      \bibinfo{booktitle}{\emph{Financial Cryptography and Data Security}}.
      \bibinfo{pages}{523–540}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Kim, Lee, Koo, Park, and Moon}{Kim
      et~al\mbox{.}}{2021}]%
            {Ethanos2021}
    \bibfield{author}{\bibinfo{person}{Jae-Yun Kim}, \bibinfo{person}{Junmo Lee},
      \bibinfo{person}{Yeonjae Koo}, \bibinfo{person}{Sanghyeon Park}, {and}
      \bibinfo{person}{Soo-Mook Moon}.} \bibinfo{year}{2021}\natexlab{}.
    \newblock \showarticletitle{Ethanos: Efficient Bootstrapping for Full Nodes on
      Account-Based Blockchain}. In \bibinfo{booktitle}{\emph{EuroSys}}.
      \bibinfo{pages}{99–113}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Kokoris-Kogias, Jovanovic, Gasser, Gailly,
      Syta, and Ford}{Kokoris-Kogias et~al\mbox{.}}{2018}]%
            {OmniledgerBootstrap}
    \bibfield{author}{\bibinfo{person}{Eleftherios Kokoris-Kogias},
      \bibinfo{person}{Philipp Jovanovic}, \bibinfo{person}{Linus Gasser},
      \bibinfo{person}{Nicolas Gailly}, \bibinfo{person}{Ewa Syta}, {and}
      \bibinfo{person}{Bryan Ford}.} \bibinfo{year}{2018}\natexlab{}.
    \newblock \showarticletitle{OmniLedger: A Secure, Scale-Out, Decentralized
      Ledger via Sharding}.
    \newblock \bibinfo{journal}{\emph{IEEE S\&P}} (\bibinfo{year}{2018}),
      \bibinfo{pages}{583--598}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Kosny and Skibski}{Kosny and Skibski}{2023}]%
            {centralityGeneral1}
    \bibfield{author}{\bibinfo{person}{Wiktoria Kosny} {and} \bibinfo{person}{Oskar
      Skibski}.} \bibinfo{year}{2023}\natexlab{}.
    \newblock \showarticletitle{Axiomatic Analysis of Medial Centrality Measures}.
      In \bibinfo{booktitle}{\emph{AAMAS}}. \bibinfo{pages}{2188–2196}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Kusmierz and Overko}{Kusmierz and
      Overko}{2022}]%
            {centralizationMetricsGeneral1}
    \bibfield{author}{\bibinfo{person}{Bartosz Kusmierz} {and}
      \bibinfo{person}{Roman Overko}.} \bibinfo{year}{2022}\natexlab{}.
    \newblock \showarticletitle{How centralized is decentralized? Comparison of
      wealth distribution in coins and tokens}. In \bibinfo{booktitle}{\emph{IEEE
      International Conference on Omni-layer Intelligent Systems (COINS)}}.
      \bibinfo{pages}{1--6}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Kwon and Buchman}{Kwon and Buchman}{[n.d.]}]%
            {cosmos}
    \bibfield{author}{\bibinfo{person}{Jae Kwon} {and} \bibinfo{person}{Ethan
      Buchman}.} \bibinfo{year}{[n.d.]}\natexlab{}.
    \newblock \bibinfo{title}{Internet of blockchains}.
    \newblock
    \newblock
    \urldef\tempurl%
    \url{v1.cosmos.network/resources/whitepaper}
    \showURL{%
    \tempurl}
    
    
    \bibitem[\protect\citeauthoryear{Kwon, Liu, Kim, Song, and Kim}{Kwon
      et~al\mbox{.}}{2019}]%
            {awesomeDecentralization}
    \bibfield{author}{\bibinfo{person}{Yujin Kwon}, \bibinfo{person}{Jian Liu},
      \bibinfo{person}{Minjeong Kim}, \bibinfo{person}{Dawn Song}, {and}
      \bibinfo{person}{Yongdae Kim}.} \bibinfo{year}{2019}\natexlab{}.
    \newblock \showarticletitle{Impossibility of Full Decentralization in
      Permissionless Blockchains}. In \bibinfo{booktitle}{\emph{ACM Conference on
      Advances in Financial Technologies}}. \bibinfo{pages}{110–123}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Leung, Suhl, Gilad, and Zeldovich}{Leung
      et~al\mbox{.}}{2019}]%
            {VaultBootstrap}
    \bibfield{author}{\bibinfo{person}{Derek Leung}, \bibinfo{person}{Adam Suhl},
      \bibinfo{person}{Yossi Gilad}, {and} \bibinfo{person}{Nickolai Zeldovich}.}
      \bibinfo{year}{2019}\natexlab{}.
    \newblock \showarticletitle{Vault: Fast Bootstrapping for the Algorand
      Cryptocurrency}. In \bibinfo{booktitle}{\emph{NDSS}}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Lin, Li, Zhao, and Chen}{Lin
      et~al\mbox{.}}{2021}]%
            {centralizationMetricsGeneral2}
    \bibfield{author}{\bibinfo{person}{Qinwei Lin}, \bibinfo{person}{Chao Li},
      \bibinfo{person}{Xifeng Zhao}, {and} \bibinfo{person}{Xianhai Chen}.}
      \bibinfo{year}{2021}\natexlab{}.
    \newblock \showarticletitle{Measuring decentralization in bitcoin and ethereum
      using multiple metrics and granularities}. In
      \bibinfo{booktitle}{\emph{International Conference on Data Engineering
      Workshops (ICDEW)}}. \bibinfo{pages}{80--87}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Liu and Zhu}{Liu and Zhu}{2022}]%
            {AirdropSybil}
    \bibfield{author}{\bibinfo{person}{Zheng Liu} {and} \bibinfo{person}{Hongyang
      Zhu}.} \bibinfo{year}{2022}\natexlab{}.
    \newblock \showarticletitle{Fighting Sybils in Airdrops}.
    \newblock \bibinfo{journal}{\emph{ArXiv}}  \bibinfo{volume}{abs/2209.04603}
      (\bibinfo{year}{2022}).
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Mazalov, Avrachenkov, Trukhina, and
      Tsynguev}{Mazalov et~al\mbox{.}}{2016}]%
            {betweennessCentralization}
    \bibfield{author}{\bibinfo{person}{Vladimir~V. Mazalov},
      \bibinfo{person}{Konstantin~E. Avrachenkov}, \bibinfo{person}{L.~I.
      Trukhina}, {and} \bibinfo{person}{Bulat~T. Tsynguev}.}
      \bibinfo{year}{2016}\natexlab{}.
    \newblock \showarticletitle{Game-Theoretic Centrality Measures for Weighted
      Graphs}.
    \newblock \bibinfo{journal}{\emph{Fundam. Informaticae}}  \bibinfo{volume}{145}
      (\bibinfo{year}{2016}), \bibinfo{pages}{341--358}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Micali, Rabin, and Vadhan}{Micali
      et~al\mbox{.}}{1999}]%
            {vrf}
    \bibfield{author}{\bibinfo{person}{Silvio Micali}, \bibinfo{person}{Michael~O.
      Rabin}, {and} \bibinfo{person}{Salil~P. Vadhan}.}
      \bibinfo{year}{1999}\natexlab{}.
    \newblock \showarticletitle{Verifiable random functions}.
    \newblock \bibinfo{journal}{\emph{40th Annual Symposium on Foundations of
      Computer Science}} (\bibinfo{year}{1999}), \bibinfo{pages}{120--130}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Momtaz}{Momtaz}{2020}]%
            {ICO2020Momtaz}
    \bibfield{author}{\bibinfo{person}{Paul~P. Momtaz}.}
      \bibinfo{year}{2020}\natexlab{}.
    \newblock \showarticletitle{Initial Coin Offerings}.
    \newblock \bibinfo{journal}{\emph{PLoS ONE}}  \bibinfo{volume}{15}
      (\bibinfo{year}{2020}).
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Nakamoto}{Nakamoto}{2009}]%
            {Nakamoto2009}
    \bibfield{author}{\bibinfo{person}{Satoshi Nakamoto}.}
      \bibinfo{year}{2009}\natexlab{}.
    \newblock \bibinfo{title}{Bitcoin : A Peer-to-Peer Electronic Cash System}.
    \newblock
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Nambiampurath}{Nambiampurath}{2023}]%
            {governanceProblem}
    \bibfield{author}{\bibinfo{person}{Rahul Nambiampurath}.}
      \bibinfo{year}{2023}\natexlab{}.
    \newblock \bibinfo{title}{Polygon receives criticism as it completes hard fork
      with only 13 validators}.
    \newblock
    \newblock
    \urldef\tempurl%
    \url{https://www.investopedia.com/polygon-receives-criticism-after-hard-fork-7096331}
    \showURL{%
    \tempurl}
    
    
    \bibitem[\protect\citeauthoryear{Narayanam and Narahari}{Narayanam and
      Narahari}{2011}]%
            {narhariCentralization}
    \bibfield{author}{\bibinfo{person}{Ramasuri Narayanam} {and}
      \bibinfo{person}{Y. Narahari}.} \bibinfo{year}{2011}\natexlab{}.
    \newblock \showarticletitle{A Shapley Value-Based Approach to Discover
      Influential Nodes in Social Networks}.
    \newblock \bibinfo{journal}{\emph{IEEE Transactions on Automation Science and
      Engineering}}  \bibinfo{volume}{8} (\bibinfo{year}{2011}),
      \bibinfo{pages}{130--147}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Narayanan, Bonneau, Felten, Miller, and
      Goldfeder}{Narayanan et~al\mbox{.}}{2016}]%
            {NarayananBitcoin}
    \bibfield{author}{\bibinfo{person}{Arvind Narayanan}, \bibinfo{person}{Joseph
      Bonneau}, \bibinfo{person}{Edward Felten}, \bibinfo{person}{Andrew Miller},
      {and} \bibinfo{person}{Steven Goldfeder}.} \bibinfo{year}{2016}\natexlab{}.
    \newblock \bibinfo{title}{Bitcoin and Cryptocurrency Technologies: A
      Comprehensive Introduction}.
    \newblock
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Platt, Sedlmeir, Platt, Xu, Tasca, Vadgama,
      and Iba{\~n}ez}{Platt et~al\mbox{.}}{2021}]%
            {energyBlockchain}
    \bibfield{author}{\bibinfo{person}{Moritz Platt}, \bibinfo{person}{Johannes
      Sedlmeir}, \bibinfo{person}{Daniel Platt}, \bibinfo{person}{Jiahua Xu},
      \bibinfo{person}{Paolo Tasca}, \bibinfo{person}{Nikhil Vadgama}, {and}
      \bibinfo{person}{Juan~Ignacio Iba{\~n}ez}.} \bibinfo{year}{2021}\natexlab{}.
    \newblock \showarticletitle{The energy footprint of blockchain consensus
      mechanisms beyond proof-of-work}. In \bibinfo{booktitle}{\emph{International
      Conference on Software Quality, Reliability and Security Companion (QRS-C)}}.
      \bibinfo{pages}{1135--1144}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Raman and Varshney}{Raman and
      Varshney}{2021}]%
            {storageCentralizationMetric}
    \bibfield{author}{\bibinfo{person}{Ravi~Kiran Raman} {and}
      \bibinfo{person}{Lav~R. Varshney}.} \bibinfo{year}{2021}\natexlab{}.
    \newblock \showarticletitle{Coding for Scalable Blockchains via Dynamic
      Distributed Storage}.
    \newblock \bibinfo{journal}{\emph{IEEE/ACM Trans. Netw.}} (\bibinfo{date}{dec}
      \bibinfo{year}{2021}), \bibinfo{pages}{2588–2601}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Rauchs and Hileman}{Rauchs and
      Hileman}{2017}]%
            {Hileman17}
    \bibfield{author}{\bibinfo{person}{Michel Rauchs} {and}
      \bibinfo{person}{Garrick Hileman}.} \bibinfo{year}{2017}\natexlab{}.
    \newblock \bibinfo{title}{Global Cryptocurrency Benchmarking Study}.
    \newblock
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Redman}{Redman}{2021}]%
            {AirdropResource1}
    \bibfield{author}{\bibinfo{person}{Jamie Redman}.}
      \bibinfo{year}{2021}\natexlab{}.
    \newblock \bibinfo{title}{Gas DAO Project Forms to Airdrop Tokens to Ethereum
      Users That Spent \$1,559 in Fees}.
    \newblock
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Roughgarden}{Roughgarden}{2020}]%
            {roughgarden2}
    \bibfield{author}{\bibinfo{person}{Tim Roughgarden}.}
      \bibinfo{year}{2020}\natexlab{}.
    \newblock \showarticletitle{Transaction fee mechanism design for the Ethereum
      blockchain: An economic analysis of EIP-1559}.
    \newblock \bibinfo{journal}{\emph{arXiv preprint arXiv:2012.00854}}
      (\bibinfo{year}{2020}).
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Roughgarden}{Roughgarden}{2021}]%
            {roughgardenTFM1}
    \bibfield{author}{\bibinfo{person}{Tim Roughgarden}.}
      \bibinfo{year}{2021}\natexlab{}.
    \newblock \showarticletitle{Transaction fee mechanism design}.
    \newblock \bibinfo{journal}{\emph{ACM SIGecom Exchanges}} \bibinfo{volume}{19},
      \bibinfo{number}{1} (\bibinfo{year}{2021}), \bibinfo{pages}{52--55}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Sai, Buckley, Fitzgerald, and Gear}{Sai
      et~al\mbox{.}}{2021}]%
            {centralizationSurvey}
    \bibfield{author}{\bibinfo{person}{Ashish~Rajendra Sai}, \bibinfo{person}{Jim
      Buckley}, \bibinfo{person}{Brian Fitzgerald}, {and}
      \bibinfo{person}{AndrewJ.~L. Gear}.} \bibinfo{year}{2021}\natexlab{}.
    \newblock \showarticletitle{Taxonomy of Centralization in Public Blockchain
      Systems: A Systematic Literature Review}.
    \newblock \bibinfo{journal}{\emph{Inf. Process. Manag.}}  \bibinfo{volume}{58}
      (\bibinfo{year}{2021}), \bibinfo{pages}{102584}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Sandor and Genc}{Sandor and Genc}{2022}]%
            {luna}
    \bibfield{author}{\bibinfo{person}{Krisztian Sandor} {and}
      \bibinfo{person}{Ekin Genc}.} \bibinfo{year}{2022}\natexlab{}.
    \newblock \bibinfo{title}{The Fall of Terra: A timeline of the meteoric rise
      and crash of UST and luna}.
    \newblock
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Schout}{Schout}{2020}]%
            {centralizationSource}
    \bibfield{author}{\bibinfo{person}{Gisele Schout}.}
      \bibinfo{year}{2020}\natexlab{}.
    \newblock \bibinfo{title}{Centralization of stake in Pos}.
    \newblock
    \newblock
    \urldef\tempurl%
    \url{medium.com/stakin/centralization-of-stake-in-pos-f7ccb8f8254}
    \showURL{%
    \tempurl}
    
    
    \bibitem[\protect\citeauthoryear{Srinivasan}{Srinivasan}{2017}]%
            {centralizationBlog}
    \bibfield{author}{\bibinfo{person}{Balaji~S Srinivasan}.}
      \bibinfo{year}{2017}\natexlab{}.
    \newblock \bibinfo{title}{Quantifying Decentralization}.
    \newblock
    \newblock
    \urldef\tempurl%
    \url{https://news.earn.com/quantifying-decentralization-e39db233c28e}
    \showURL{%
    \tempurl}
    
    
    \bibitem[\protect\citeauthoryear{Sultanik, Remie, Manzano, Brunson, Moelius,
      Kilmer, Myers, Amir, and Schriner}{Sultanik et~al\mbox{.}}{2022}]%
            {DecentralizationTrailofBits}
    \bibfield{author}{\bibinfo{person}{Evan Sultanik}, \bibinfo{person}{Alexander
      Remie}, \bibinfo{person}{Felipe Manzano}, \bibinfo{person}{Trent Brunson},
      \bibinfo{person}{Sam Moelius}, \bibinfo{person}{Sam Kilmer},
      \bibinfo{person}{Mike Myers}, \bibinfo{person}{Talley Amir}, {and}
      \bibinfo{person}{Sonya Schriner}.} \bibinfo{year}{2022}\natexlab{}.
    \newblock \showarticletitle{Are blockchains decentralized? Unintended
      centralities in distributed ledgers}.
    \newblock \bibinfo{journal}{\emph{Trail of Bits}} (\bibinfo{year}{2022}).
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Waniek, Wo\'{z}nica, Zhou, Vorobeychik,
      Rahwan, and Michalak}{Waniek et~al\mbox{.}}{2021}]%
            {centralizationSecurity}
    \bibfield{author}{\bibinfo{person}{Marcin Waniek}, \bibinfo{person}{Jan
      Wo\'{z}nica}, \bibinfo{person}{Kai Zhou}, \bibinfo{person}{Yevgeniy
      Vorobeychik}, \bibinfo{person}{Talal Rahwan}, {and}
      \bibinfo{person}{Tomasz~P. Michalak}.} \bibinfo{year}{2021}\natexlab{}.
    \newblock \showarticletitle{Strategic Evasion of Centrality Measures}. In
      \bibinfo{booktitle}{\emph{AAMAS}}. \bibinfo{pages}{1389–1397}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{W\k{a}s, Waniek, Rahwan, and Michalak}{W\k{a}s
      et~al\mbox{.}}{2020}]%
            {centralitySecurity2}
    \bibfield{author}{\bibinfo{person}{Tomasz W\k{a}s}, \bibinfo{person}{Marcin
      Waniek}, \bibinfo{person}{Talal Rahwan}, {and} \bibinfo{person}{Tomasz
      Michalak}.} \bibinfo{year}{2020}\natexlab{}.
    \newblock \showarticletitle{The Manipulability of Centrality Measures-An
      Axiomatic Approach}. In \bibinfo{booktitle}{\emph{AAMAS}}.
      \bibinfo{pages}{1467–1475}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Wood}{Wood}{2014}]%
            {wood2014ethereum}
    \bibfield{author}{\bibinfo{person}{Gavin Wood}.}
      \bibinfo{year}{2014}\natexlab{}.
    \newblock \showarticletitle{Ethereum: A secure decentralised generalised
      transaction ledger}.
    \newblock \bibinfo{journal}{\emph{Ethereum project yellow paper}}
      \bibinfo{volume}{151} (\bibinfo{year}{2014}), \bibinfo{pages}{1--32}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Wu, Peng, Xie, and Huang}{Wu
      et~al\mbox{.}}{2019}]%
            {entropyDecentralization}
    \bibfield{author}{\bibinfo{person}{Keke Wu}, \bibinfo{person}{Bo Peng},
      \bibinfo{person}{Hua Xie}, {and} \bibinfo{person}{Zhen Huang}.}
      \bibinfo{year}{2019}\natexlab{}.
    \newblock \showarticletitle{An Information Entropy Method to Quantify the
      Degrees of Decentralization for Blockchain Systems}.
    \newblock \bibinfo{journal}{\emph{International Conference on Electronics
      Information and Emergency Communication (ICEIEC)}} (\bibinfo{year}{2019}),
      \bibinfo{pages}{1--6}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Xiao, Zhang, Lou, and Hou}{Xiao
      et~al\mbox{.}}{2020}]%
            {consensusSurvey}
    \bibfield{author}{\bibinfo{person}{Yang Xiao}, \bibinfo{person}{Ning Zhang},
      \bibinfo{person}{Wenjing Lou}, {and} \bibinfo{person}{Y.~Thomas Hou}.}
      \bibinfo{year}{2020}\natexlab{}.
    \newblock \showarticletitle{A Survey of Distributed Consensus Protocols for
      Blockchain Networks}.
    \newblock \bibinfo{journal}{\emph{IEEE Communications Surveys \& Tutorials}}
      \bibinfo{volume}{22} (\bibinfo{year}{2020}), \bibinfo{pages}{1432--1465}.
    \newblock
    
    
    \bibitem[\protect\citeauthoryear{Zhang, Xue, and Liu}{Zhang
      et~al\mbox{.}}{2019}]%
            {securitySurvey}
    \bibfield{author}{\bibinfo{person}{Rui Zhang}, \bibinfo{person}{Rui Xue}, {and}
      \bibinfo{person}{Ling Liu}.} \bibinfo{year}{2019}\natexlab{}.
    \newblock \showarticletitle{Security and Privacy on Blockchain}.
    \newblock \bibinfo{journal}{\emph{ACM Comput. Surv.}} (\bibinfo{date}{jul}
      \bibinfo{year}{2019}).
    \newblock
    
    
    \end{thebibliography}
  
